Fast Stencil Computations using Fast Fourier Transforms

Stencil computations are widely used to simulate the change of state of physical systems across a multidimensional grid over multiple timesteps. The state-of-the-art techniques in this area fall into three groups: cache-aware tiled looping algorithms, cache-oblivious divide-and-conquer trapezoidal algorithms, and Krylov subspace methods. In this paper, we present two efficient parallel algorithms for performing linear stencil computations. Current direct solvers in this domain are computationally inefficient, and Krylov methods require manual labor and mathematical training. We solve these problems for linear stencils by using DFT preconditioning on a Krylov method to achieve a direct solver which is both fast and general. Indeed, while all currently available algorithms for solving general linear stencils perform $\Theta(NT)$ work, where $N$ is the size of the spatial grid and $T$ is the number of timesteps, our algorithms perform $o(NT)$ work. To the best of our knowledge, we give the first algorithms that use fast Fourier transforms to compute final grid data by evolving the initial data for many timesteps at once. Our algorithms handle both periodic and aperiodic boundary conditions, and achieve polynomially better performance bounds (i.e., computational complexity and parallel runtime) than all other existing solutions. Initial experimental results show that implementations of our algorithms that evolve grids of roughly $10^7$ cells for around $10^5$ timesteps run orders of magnitude faster than state-of-the-art implementations for periodic stencil problems, and 1.3$\times$ to 8.5$\times$ faster for aperiodic stencil problems.

==> OLD-experiments.tex <==
\section{Experiments}
In this section, we present the experimental evaluation of our algorithms comparing with the state-of-the-art stencil algorithms. We also provide scalability results of our implementations.

\paragraph{Experimental Setup.}
All experiments were performed on Knights Landing (KNL) Intel Xeon Phi 7250 nodes of Stampede2 Supercomputer \cite{Stampede2}. Each node has 68 cores and 272 hardware threads (4 threads per core) on a single socket. Each KNL node has 32 KB L1 data cache per core, 1 MB L2 cache per two-core tile, 16 GB direct-mapped L3 cache, and a 96 GB DDR4 RAM.

All algorithms were implemented in C++. We used Intel C++ Compiler (ICC) v18.0.2 with \texttt{gnu++98} standard to compile our implementations with the optimization parameters \texttt{-O3 -xhost -ansi-alias -ipo -AVX512}. We used OpenMP 5.0 with ICC for our shared-memory parallel implementations. The threads were pinned to CPU cores using \texttt{GOMP\_CPU\_AFFINITY}.

\paragraph{Benchmarks and Problem Sizes.} We implemented heat equations with both periodic and aperiodic boundary conditions. Table \ref{tab:problem-sizes} shows the problem sizes for our benchmarks.

\begin{table}[!ht]
\centering
\scalebox{0.8}{
\begin{colortabular}{ | c | c | c | c|}
\hline                       

Problem & $N$ & $T$ & MSE (for $T = 1000$) \\ \hline

\texttt{heat1d} & $1,600,000$ & $[10^3, 10^9]$ & $5.55291\times 10^{-24}$\\
\texttt{heat2d} & $8,000 \times 8,000 $ & $[10^1, 10^9]$ & $2.24553\times10^{-21}$\\
%\texttt{heat-3d} & & \\
\texttt{heat3d} & $300 \times 300 \times 300 $ & $[10^1, 10^9]$ & $1.49097\times10^{-21}$\\


\end{colortabular}
}
\tabcaption{Problem sizes. Here, MSE = mean square error.}
\label{tab:problem-sizes}
\vgap{}\vgap{}\vgap{}\vgap{}
\end{table}

\begin{figure*}[!ht]
\begin{minipage}{\textwidth}
\begin{minipage}{0.33\textwidth}
\centering
\includegraphics[width=\textwidth]{runtime-periodic-heat1d.pdf}\\
$(a)$
\end{minipage}
\begin{minipage}{0.33\textwidth}
\centering
\includegraphics[width=\textwidth]{runtime-periodic-heat2d.pdf}\\
$(b)$
\end{minipage}
\begin{minipage}{0.33\textwidth}
\centering
\includegraphics[width=\textwidth]{scaling-periodic-heat.pdf}\\
$(e)$
\end{minipage}
\end{minipage}
\begin{minipage}{\textwidth}
\begin{minipage}{0.33\textwidth}
\centering
\includegraphics[width=\textwidth]{runtime-periodic-heat3d.pdf}\\
$(c)$
\end{minipage}
\begin{minipage}{0.33\textwidth}
\centering
\includegraphics[width=\textwidth]{runtime-aperiodic-heat1d.pdf}\\
$(d)$
\end{minipage}
\begin{minipage}{0.33\textwidth}
\centering
\includegraphics[width=\textwidth]{scaling-aperiodic-heat.pdf}\\
$(f)$
\end{minipage}
\vgap{}
\caption{Plots $a-d$ show the performance comparison of our FFT-based stencil algorithms with state-of-the-art parallel tiled algorithms for $(a,b,c)$ periodic \texttt{heat1d}, \texttt{heat2d}, and \texttt{heat3d}, and $(d)$ iterative aperiodic \texttt{heat1d} (see Section~\ref{iter-aperiodic-alg}). Plots $e$ and $f$ show the scalability analysis of our FFT-based stencil algorithms for $(e)$ periodic \texttt{heat1d}, \texttt{heat2d}  and \texttt{heat3d} and $(f)$ aperiodic \texttt{heat1d}, when the number of cores $p$ is varied. For all plots, the problem sizes are given in Table \ref{tab:problem-sizes}.}
\label{fig:runtimes}
\end{minipage}
\vspace{0.2cm}

\begin{minipage}{\textwidth}
\centering
\begin{colortabular}{ | l | l | r | r | r | r | r | r |}
\hline                       

\multicolumn{2}{l|}{Benchmark} & \multicolumn{2}{c|}{Tiled algorithms (68 cores)} & \multicolumn{2}{c|}{Our FFT-based algorithms} & \multicolumn{2}{|c|}{Speedup over} \\
\rowcolor{tabletitlecolor} \multicolumn{2}{c|}{} & \texttt{standard} & \texttt{diamond} & \texttt{serial} & \texttt{parallel} & \texttt{standard} & \texttt{diamond} \\\hline

\multirow{2}{*}{Periodic} & \texttt{heat1d} $(T = 10^7)$ & $>5000$ & $\phantom{>}789$ & 0.268 & 0.048 (16 cores) & $>$ 100000 & 16444 \\

& \texttt{heat2d} $(T = 10^5)$ & $\phantom{>}1597$ & 1437 & 12.239 & 3.685 (32 cores) & 433 & 390 \\
& \texttt{heat3d} $(T = 10^5)$ & $>9000$ & 4920 & 5.244 & 2.999 (16 cores) & $>3000$ & 1645 \\\hline
%& \texttt{heat-3d} $(T = )$ & & & & & & \\ \hline
Aperiodic & \texttt{heat1d} $(T = 10^5)$ & $\phantom{>50}89$ & 113 & 8.947 & 1.555 (16 cores) & 57 & 73
\end{colortabular}
\vgap{}
\caption{Summary of performance of stencil algorithms in seconds. Here, \texttt{standard} = \texttt{pluto-standard}, and \texttt{diamond} = \texttt{pluto-diamond}. The problem sizes are given in Table \ref{tab:problem-sizes}.}
\vspace{-0.3cm}
\label{tab:experimental-results}
\end{minipage}
\end{figure*}

\paragraph{PLuTo-Generated Stencil Programs.} The tiled looping implementations were generated by PLuTo \cite{Pluto} -- the state-of-the-art tiled looping code generator. The two main types of tiling methods used for performance comparison are: \texttt{pluto-standard} and \texttt{pluto-diamond}, whose tiles have the shapes of parallelograms and diamonds, respectively. \hide{The \texttt{pluto-diamond} algorithm exploits better data locality and achieves better scaling than \texttt{pluto-standard} \cite{bondhugula2017}.} These parallel implementations were run on 68 cores. The tile sizes were selected for these implementations via a small autotuning phase, exploring sizes from $\{ 8, 16, 32\}$ for the outer dimensions and from $\{64, 128, 512\}$ for the inner-most dimension to ensure that enough multithread parallelism was exposed in the wavefront dimension created by PLuTo, while ensuring the tile footprint neared the cache size.

\paragraph{Our FFT-Based Stencil Programs.}
We implemented our FFT-based stencil algorithms making use of the shared-memory FFT implementation from Intel Math Kernel Library (Intel MKL) \cite{MKL} for 1-D and FFTW3 \cite{frigo2005design} for 2-D and 3-D. We implemented a simpler version of our aperiodic algorithm, i.e., iterative aperiodic algorithm (see Section \ref{iter-aperiodic-alg}). Our implementations are available at \texttt{https://bit.ly/FastStencil-FFT}. 

\hide{
\paragraph{Number of Timesteps.} In the literature, stencil computations are usually performed for a few hundreds of timesteps. In our experiments, we vary the number of timesteps $T$ from a few thousands to very large values. The motivation for simulating stencil computations for large number of timesteps is as follows: $(i)$ the state of a big physical system (e.g. fluid dynamics) might change quickly which necessitates simulations over a large number of tiny timesteps, $(ii)$ quick simulations of stencil computations over large number of timesteps can help us to iteratively improve our initially chosen stencil to realistically model the real-world, and $(iii)$ rules (or stencils) in problems such as \textit{game of life} will not change over time and hence can be used for simulating a large number of timesteps. 
}

\paragraph{Performance Analysis.} Figures \ref{fig:runtimes} $(a,b,c,d)$ and \ref{tab:experimental-results} show the performance comparison of the implementations of our algorithms with \texttt{pluto-standard} and \texttt{pluto-diamond}. The two FFT-based implementations shown in the plots are:\\ \texttt{fft-serial} -- a serial version, and \texttt{fft-par16} or \texttt{fft-par32} -- parallel versions using 16 and 32 threads, respectively. The best parallel implementations of our algorithms run 390$\times$ to 16,444$\times$ faster than the best existing codes (generated by PLuTo \cite{Pluto}) for periodic stencils and 57$\times$ faster for aperiodic stencils. Observe that the speedups of our periodic stencil codes over the tiled loop counterparts will keep increasing at approximately the same rate as $T$ for larger grid sizes.

Please note that our recursive aperiodic algorithm described in Section \ref{sec:aperiodic} is much more efficient than the iterative aperiodic algorithm we have implemented for our experiments. We believe that the implementation of our recursive algorithm will lead to better speedups.

\paragraph{Scalability Analysis.} Our algorithms are highly parallel and should scale accordingly. However, we use FFT computations that are memory bound -- they perform only $\Th{n\log{n}}$ work on an input of size $\Th{n}$ and thus have very little data reuse\footnote{which is evident from their (optimal) $\Oh{\frac{n}{B}\log_{M}{n}}$ cache complexity with a low temporal locality}. 
As a result, our programs may slow down with the increase of the number of concurrent threads when the memory bandwidth is low. Indeed, we observe that the \texttt{forward} and \texttt{backward} FFT computations are the scalability bottlenecks of our algorithms. Figure \ref{fig:runtimes} $(e,f)$ shows the scalability plots for our implementations, where $T = 10^9$ and $T = 10^6$ for plots $(e)$ and $(f)$, respectively.

\paragraph{Numerical Accuracy.} We validated our results by comparing with the output from the standard na\"ive iterative looping implementations. As the looping implementations were slow, we computed the mean square error (MSE) for 1000 timesteps. Table \ref{tab:problem-sizes} summarizes MSE for our benchmarks.

